Tooling Offline Runtime Verification against Interaction Models : recognizing sliced behaviors using parameterized simulation

Offline runtime verification involves the static analysis of executions of a system against a specification. For distributed systems, it is generally not possible to characterize executions in the form of global traces, given the absence of a global clock. To account for this, we model executions as collections of local traces called multi-traces, with one local trace per group of co-localized actors that share a common clock. Due to the difficulty of synchronizing the start and end of the recordings of local traces, events may be missing at their beginning or end. Considering such partially observed multi-traces is challenging for runtime verification. To that end, we propose an algorithm that verifies the conformity of such traces against formal specifications called Interactions (akin to Message Sequence Charts). It relies on parameterized simulation to reconstitute unobserved behaviors.

==> figures/2_multitrace/subfig/tikz_l1.tex <==
\begin{tikzpicture}[every node/.style={minimum height=0pt,minimum width=0pt,inner sep=0,outer sep=0}]
    \node (lab) {$\hlf{l_1}$};
    \node[below=-.4cm of lab] (img) {\includegraphics[height=.9cm]{images/icons/icon_laptop_v3.png}};
\end{tikzpicture}

==> figures/2_multitrace/subfig/tikz_l2.tex <==
\begin{tikzpicture}[every node/.style={minimum height=0pt,minimum width=0pt,inner sep=0,outer sep=0}]
    \node (img) {\includegraphics[width=.9cm]{images/icons/icon_device.png}};
    \node[below right=-.3cm and -.4cm of img] (lab) {$\hlf{l_2}$};
\end{tikzpicture}

==> figures/2_multitrace/subfig/tikz_l3.tex <==
\begin{tikzpicture}[every node/.style={minimum height=0pt,minimum width=0pt,inner sep=0,outer sep=0}]
    \node (img) {\includegraphics[width=.9cm]{images/icons/icon_cog_belt.png}};
    \node[below left=-.6cm and -.5cm of img] (lab) {$\hlf{l_3}$};
\end{tikzpicture}
